Learning Goals from Failure

We introduce a framework that predicts the goals behind observable human action in video. Motivated by evidence in developmental psychology, we leverage video of unintentional action to learn video representations of goals without direct supervision. Our approach models videos as contextual trajectories that represent both low-level motion and high-level action features. Experiments and visualizations show our trained model is able to predict the underlying goals in video of unintentional action. We also propose a method to "automatically correct" unintentional action by leveraging gradient signals of our model to adjust latent trajectories. Although the model is trained with minimal supervision, it is competitive with or outperforms baselines trained on large (supervised) datasets of successfully executed goals, showing that observing unintentional action is crucial to learning about goals in video. Project page: https://aha.cs.columbia.edu/

==> ac_tables.tex <==
%\begin{wraptable}{R}{.6\textwidth}
\begin{table}[t]
% \begin{table}[tb]
\centering
% \resizebox{0.55\linewidth}{!}{
\resizebox{\columnwidth}{!}{
\begin{tabular}{c l|c c c c c c}
\toprule
% && \multicolumn{2}{c|}{\textbf{Localization within}} & \textbf{Classification} \\
% && \multicolumn{4}{c|}{\textbf{Autocorrect Statistics}} & \multicolumn{4}{c}{\textbf{$\Delta$ SVO Prediction}} \\
&\textbf{Method} & \textbf{No. iters} & \textbf{Success @ 25} & \textbf{@10} & \textbf{$\mathbf{\Delta}$ Acc.} & \textbf{$\mathbf{\Delta \mathcal{L}_{nsp}}$} \\ \midrule
&Kinetics 3D \cite{carreira2017quo} & 16.81 & 92.92 & 31.60 & - & - \\
&3D CNN only \cite{oops}  & 8.35 & 93.24 & 91.05 & - & - \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Our model}} & Classification only & 12.19 & 93.24 & 55.72 & +4.15 & - \\
&   + Pseudo-GT  & 12.91 & 93.24 & 47.97 & +4.64 & - \\
&   + Coherence loss  & 11.87 & 93.24 & 59.17 & +8.84 & -0.1521 \\
&    \quad + Pseudo-GT & 12.74 & 93.24 & 49.12 & +2.69 & -0.0713  \\ \bottomrule
\end{tabular}
}
% }
% \vspace{0.5em}
\caption{\textbf{Evaluating autocorrect:} We show information on the auto-correct process, including how many iterations it requires to converge and the increase in accuracy it causes in classification of {\em pre-failure} intentional action and of temporal coherence, which we hypothesize is due to the decreased entropy of intentional action. Results suggest that there is a subset of videos that are not correctable by our process, since success at 25 iterations is fixed across all models.}
\label{tbl:ac_stats_eval}  
% \vspace{-2em}
% \end{table}
%\end{wraptable}
\end{table}
